Deep Temporal Interpolation of Radar-based Precipitation

When providing the boundary conditions for hydrological flood models and estimating the associated risk, interpolating precipitation at very high temporal resolutions (e.g. 5 minutes) is essential not to miss the cause of flooding in local regions. In this paper, we study optical flow-based interpolation of globally available weather radar images from satellites. The proposed approach uses deep neural networks for the interpolation of multiple video frames, while terrain information is combined with temporarily coarse-grained precipitation radar observation as inputs for self-supervised training. An experiment with the Meteonet radar precipitation dataset for the flood risk simulation in Aude, a department in Southern France (2018), demonstrated the advantage of the proposed method over a linear interpolation baseline, with up to 20% error reduction.

==> demo.tex <==
\section{Impact Analysis}

To demonstrate the impact of various precipitation interpolation methods in flood simulation with IFM, we selected an actual flooding event in the past.  We select a flooding event in Aude, France back in October, 2018.  ``Several months' worth of rain fell within a few hours overnight in Aude, leaving people stranded on rooftops'', according to a news article by Sky News. In this event, a number of flash floods has been reported that typically be driven by heavy rainfall in a short period so requiring high resolution rainfall information in space and time to analyze the details using hydrological models.


\subsection{Historical Events}

A total of 8 historical flooding events, from various locations across the globe were selected for the validation analysis (Table 1). All the flooding events where a result of extreme and often short-lived rainfall phenomenon, such as hurricanes, or other extreme weather systems. Table 1 provides a summary of the events, as well as the details of the model simulations. 

\begin{table}
	\caption{Events used in the validation}
	
\end{table}

\begin{figure*}[hbt]
  \centering
  \includegraphics[width=1.0\textwidth]{images/0172800_binary.pdf}
  \caption{Flooding simulation results at timestamp 2018-10-16 00:00:00 using input precipitation from the original fine temporal resolution (5 minutes interval, left) and from the linear interpolation (from 60 minutes to 5 minutes interval, middle). For illustration, a water depth threshold of 0.15\,m is used to define a pixel as flooded. The absolute difference of the two flood distribution (right) is mapped in colors (red - missing, blue - extra).}
  \label{fig:ifm_48h}
\end{figure*}

We applied various temporal resolution of precipitation made from the MeteoNet dataset, 5-min resolution as is and half-hourly resolution by under-sampling.  While the interpolation has been applied in the overall area (South-East of France) of Meteonet, the evaluation is focused around Aude, a bounding rectangle where geographical coordinates of southwest and northeast corners in latitude and longitude are (43.1161, 2.8717) and (43.3218, 3.1795), respectively, so that major observed flash floods are included in the region of our analysis. For comparison, we also obtained simple linear interpolation results with the same setting as above. The interpolated precipitation was also used to drive the IFM and flood depth was calculated as outputs of the simulation.

Figure~\ref{fig:ifm_48h} shows the simulated flood extents at a single time stamp 48\,hours after the start of the simulation, obtained using precipitation data from both raw 5\,minutes resolution and 60-to-5\,minutes linearly interpolated resolution. The difference between these two binary maps, as shown on the right, reveals the difference in flood distribution, demonstrating the sensitivity of the flood model to the precipitation input data.

\begin{figure}[hbt]
  \centering
  \includegraphics[width=0.45\textwidth]{images/rmse_precip_flood.pdf}
%  \caption{Deviations in precipitation between the original 5 minutes resolution and the 60-to-5 minutes linearly interpolated resolution are shown by calculating the normalised root mean square error (RMSE) across the whole region of interest at each time step. The resulting impact on flooding is shown likewise by calculating the RMSE between the respectively simulated water depth maps. Note that the RMSE for flood is missing in the beginning because of too small water depths.}
  \caption{Deviations in precipitation between the original 5 minutes resolution and the 60-to-5 minutes linearly interpolated resolution.}
  \label{fig:rmse_precip_flood}
\end{figure}

In order to quantify the difference in the two precipitation data sets as well as in the resulting water depths, the root mean square errors (RMSE) are calculated across the whole area.
Figure~\ref{fig:rmse_precip_flood} shows their normalised value over the whole time of the simulation period.It can be observed that the RMSE of the flooding results becomes maximum when the difference in precipitation becomes maximum. While the RMSE in precipitation is transient, the flooding depth is affected in the longer term, with a significant error remaining even after several days at the end of the simulation period. 

These results suggest that the difference of the interpolation methods applied to precipitation that drives hydrological models has potentially considerable impact to the flood simulation results, particularly in the case of flash floods that caused by local heavy rainfalls.





==> methodology.tex <==
\section{Methodology}

Given two precipitation estimation inputs $I_0$ and $I_1$ and a time $t \in (0, 1)$, our goal is to predict the intermediate precipitation $\hat{I}$ at time
$T = t$.
In this paper we leverage an approach introduced by SuperSloMo~\cite{Jiang+:CVPR18:SuperSloMo}, a high-quality variable-length multi-frame interpolation method that can interpolate a video frame at any arbitrary time step between two frames, amongst many existing work on optical flow~\cite{Tu+:2019:CNN_optflow,Zhai+:2021:opticalflow_survey}.  
While the simple application of SuperSloMo to satellite imagery has been recently studied~\cite{Vandal+Nemani:2021:SSM_satellite}, we extend it for the purpose of precipitation interpolation and the realistic availability of supplemental data of geography.

% topography



\subsection{Training}

Reconstruction loss
Perceptual loss (n/a)
Warping loss
Smoothness loss




\subsection{Topographical }





A straightforward way is to accomplish this is to
train a neural network [16] to directly output the RGB pix-
els of Iˆ . In order to do this, however, the network has to t
learn to interpret not only the motion pattens but also the appearance of the two input images. Due to the rich RGB color space, it is hard to generate high-quality intermediate images in this way. Inspired by [1] and recent advances in single intermediate video frame interpolation [19, 20, 15], we propose fusing the warped input images at time T = t.

Let Ft→0 and Ft→1 denote the optical flow from It to I0
and It to I1, respectively. If these two flow fields are known,
we can synthesize the intermediate image Iˆ as follows: t
Iˆ =α ⊙g(I ,F )+(1−α )⊙g(I ,F ), (1) t00t→0 01t→1
where g(·, ·) is a backward warping function, which can be
implemented using bilinear interpolation [40, 15] and is differentiable. The parameter α0 controls the contribution of
the two input images and depend on two factors: temporal
consistency and occlusion reasoning. ⊙ denotes element-
wise multiplication, implying content-aware weighting of
input images. For temporal consistency, the closer the time
step T = t is to T = 0, the more contribution I0 makes to
Iˆ ; a similar property holds for I . On the other hand, an t1
important property of the video frame interpolation prob- lem is that if a pixel p is visible at T =t, it is most likely at least visible in one of the input images,1 which means the occlusion problem can be addressed. We therefore introduce visibility maps Vt←0 and Vt←1. Vt←0(p) ∈ [0, 1] denotes whether the pixel p remains visible (0 is fully occluded) when moving from T = 0 to T = t. Combining the temporal consistency and occlusion reasoning, we have


==> motivation.tex <==
% Motivation and Problem setting
\section{Motivation with Climate Impact Modeling}

\subsection{Flood Impact Models}

Climate change and variability is expected to exacerbate the occurrence and intensity of extreme weather and climate events. In response to climate change and the increasing need of optimizing and enhancing the accuracy of climate impact models, we use a system and methods that accelerate this type of climate impact and hazard modelling according to user-specified and/or learned requirements, called Climate Impact Modelling Framework (CIMF). Using this system, a user can run modularized and scalable workflows in the cloud computing environment for any impact model, with a high-level of customization and intelligent automation. For example, through CIMF models related to flood inundation can be linked to cloud-based data resources, computing resources and information delivery platforms. This allows easy and timely execution of models to map climate related natural disasters, in-order to improve emergency response management. 

Floods, which have a severe impact on nature and human society, are one of the key climate related disasters that are being considered for CIMF. Enhancing our understanding of occurrence and propagation of floods will play a role in mitigating the impact thereof. Currently CIMF, includes an onboarded pluvial flood inundation model called Integrated Flood Model (IFM)~\cite{Singhal+:EuroPar2014:IFM}. IFM is a 2D rainfall runoff model, coupled to a land-surface model. IFM allows simple execution of various model configurations, and easy scalability in the cloud. IFM is designed to model overland flow of water, driven by topographical gradients and rainfall, at various temporal and spatial resolutions. IFM and its outputs allow the easy mapping of flash floods, as well as the slow seasonal rise of water levels in catchment over a season, both in terms of extent and depth. For example, IFM can be driven through atmospheric forcing from forecasted extreme rainfall events. This would potentially hazardous events to be predicted and effective mitigation solutions put in place. 

Physical flooding simulation models similar to IFM, while potentially offering better impact prediction than simple statistical models in unseen situations, need calibration of parameters.  For example, we should adjust flood plain friction (i.e. Manning's roughness coefficients) and infiltration drainage simulation, which is derived from categorically-defined land surface parameters, based on historical flooding events.  Also, we should refine geographical elevation models originally given as 30m or even 250m resolutions, which are slightly short for capturing flooding thresholds at small banks.

%\begin{figure}[hbt]
%	\centering
%	\includegraphics[width=0.40\textwidth]{images/ifm-system.pdf}
%	\caption{The overland flooding simulation system illustration extracted from a paper on IFM~\cite{Singhal+:EuroPar2014:IFM}.  As well as terrain information, the system consumes precipitation as its input to produce flooding (water height) results for each timestamp.}
%	\label{fig:ifm-system}
%\end{figure}

\subsection{Precipitation Observation from Satellites}

%Interpolation with CHIRPS~\cite{Funk+:2015:CHIRPS}

Precipitation is one of the main causes of fatal natural disasters, as it causes flooding, landslides, and snow avalanches, for example, and also damages crops. The frequency and severity of these events is increasing with the increase in extreme weather events associated with acute climate change. Mathematical and computational models have become widely used tools to predict and mitigate risks to socioeconomic systems. However, for these predictions to be accurate, the underlying precipitation data driving the simulations have to be well resolved in space and time. 

While there are areas of the world that have dense ground-based sensors for measuring precipitation in the form of rain gauges and radars, the vast oceans, less populated regions, and parts of developing countries lack adequate surface measurements of precipitation (Kidd et al. 2017). Satellites provide an optimal platform from which to measure precipitation globally.

The Global Precipitation Measurement Core Observatory (GPM CO) spacecraft is an advanced successor to TRMM, with additional channels on a dual-frequency precipitation radar and on the microwave imager with capabilities to sense light rain and falling snow.
% (Houet al. 2008, 2014)
The GPM CO, in a NASA–JAXA partnership, was launched in February 2014 and operates in a non-sun-synchronous orbit with an inclination angle of 65°. This orbit allows the GPM CO to sample precipitation across all hours of the day from the tropics to the Arctic and Antarctic circles and for observing hurricanes and typhoons as they transition from the tropics to the midlatitudes.

IMERG data values are based on a single microwave snapshot during its half-hour analysis period, or a morphed/Kalman filter interpolation if no microwave values are available.  The values are expressed in the intensive units mm/hr, which is usually assumed that this rate applies for the entire half-hour period.
%If you wish to regrid to a finer time and/or space grid, note that many interpolation schemes have the property of suppressing maxima in precipitation and expanding rain events into neighboring zero-amount periods, so it is critical that you examine this issue and state what scheme was used in documentation and papers. 

==> relatedwork.tex <==
%
% relatedwork.tex
%
\section{Related Work}

% Wikipedia:
% A landform is a natural or artificial feature of the solid surface of the Earth or other planetary body. Landforms together make up a given terrain, and their arrangement in the landscape is known as topography. Landforms include hills, mountains, plateaus, canyons, and valleys, as well as shoreline features such as bays, peninsulas, and seas,[citation needed] including submerged features such as mid-ocean ridges, volcanoes, and the great ocean basins.

%The short term forecast is as old as weather forecasting itself. During the nineteenth century, the first modern meteorologists were using extrapolation methods for predicting the movement of low pressure systems and anticyclones on surface maps. The researchers subsequently applied the laws of fluid dynamics to the atmosphere and developed the NWP as we know it today. However, the data resolution and parameterization of meteorological primitive equations still leave uncertainty about the small-scale projections, in time and space.

Forecasting precipitation at very high resolutions in space and time, particularly with the aim of providing the boundary conditions for hydrological models and estimating the associated risk, is one of the most difficult challenges in meteorology. In short, the problem is to predict the field of precipitation on grids of 1 km or less and for horizons of less than an hour. Due to the high spatial resolutions required, methods based on meteorological models are not effective, because they are too onerous computationally and the time to perform a simulation is usually excessively too long for operational purposes. They also depend, in a critical way, on the initial conditions as the level of uncertainty is too high and it is difficult to assimilate locally recorded data. Even if these difficulties were overcome, a fundamental difficulty would remain, the gap between the spatial scales provided by the meteorological models and those useful to hydrologists for operational purposes. To overcome this difficulty and quantify the uncertainty involved, probabilistic approaches were proposed~\cite{Marrocu+Luca:Forecasting:2020}.

%Optical flow based Nowcasting~\cite{Bechini+Chandrasekar:2017:Nowcasting}.


%Topographic feature learning~\cite{Proulx-Bourque+:IGARSS2018:topographic_feature}.
